Automatic Synthesis of Random Generators for Numerically Constrained Algebraic Recursive Types

In program verification, constraint-based random testing is a powerful technique which aims at generating random test cases that satisfy functional properties of a program. However, on recursive constrained data-structures (e.g., sorted lists, binary search trees, quadtrees), and, more generally, when the structures are highly constrained, generating uniformly distributed inputs is difficult. In this paper, we present Testify: a framework in which users can define algebraic data-types decorated with high-level constraints. These constraints are interpreted as membership predicates that restrict the set of inhabitants of the type. From these definitions, Testify automatically synthesises a partial specification of the program so that no function produces a value that violates the constraints (e.g. a binary search tree where nodes are improperly inserted). Our framework augments the original program with tests that check such properties. To achieve that, we automatically produce uniform random samplers that generate values which satisfy the constraints, and verifies the validity of the outputs of the tested functions. By generating the shape of a recursive data-structure using Boltzmann sampling and generating evenly distributed finite domain variable values using constraint solving, our framework guarantees size-constrained uniform sampling of test cases. We provide use-cases of our framework on several key data structures that are of practical relevance for developers. Experiments show encouraging results.

==> appendice.tex <==
\section{BST: Constructive Approach is not Uniform\label{bstnonuniform}}
Inserting a node $n$ consists in recursively inserting $n$ to the
left subtree if its key is less than that of the root or to the
right subtree otherwise. New keys are always inserted in leaf
position. Figure~\ref{fig:nonu} shows that building trees by
generating a random sequence of insertions favours the apparition
on some values rather than others, namely the tree obtained in
figure~\ref{fig:morefrequent}.

\begin{figure}[h]
    \centering
    \subfloat[\centering Insertion order: 1,2,3]{
    \begin{forest}
for tree={
    grow=south,
    circle, draw, minimum size=3ex, inner sep=1pt,
    s sep=7mm
        }
    [1[,no edge, draw=none][2 [,no edge, draw=none] [3]]]
\end{forest}}%
    \qquad
    \centering
    \subfloat[\centering Insertion order: 1,3,2]{
    \begin{forest}
    for tree={
    grow=south,
    circle, draw, minimum size=3ex, inner sep=1pt,
    s sep=7mm
    }
    [1 [,no edge, draw=none] [3 [2] [,no edge, draw=none]]]
\end{forest}}%
    \qquad
    \centering
    \subfloat[\centering Insertion order: 2,1,3 \& 2,3,1\label{fig:morefrequent}]{
\begin{forest}
for tree={
    grow=south,
    circle, draw, minimum size=3ex, inner sep=1pt,
    s sep=7mm
        }
        [2 [1] [3]]
\end{forest}}%
    \qquad
    \centering
    \subfloat[\centering Insertion order: 3,2,1]{
\begin{forest}
for tree={
    grow=south,
    circle, draw, minimum size=3ex, inner sep=1pt,
    s sep=7mm
        }
    [3 [2 [1][,no edge, draw=none]][,no edge, draw=none]]
\end{forest}}%
    \qquad
    \centering
    \subfloat[\centering Insertion order: 3,1,2]{
\begin{forest}
for tree={
    grow=south,
    circle, draw, minimum size=3ex, inner sep=1pt,
    s sep=7mm
        }
    [3 [1[,no edge, draw=none][2]][,no edge, draw=none]]
\end{forest}}
\caption{All possible BST of size three with values: $\{1,2,3\}$}
\label{fig:nonu}
\end{figure}

\section{Generated code for BST\label{gencodebst}}
\begin{figure}[h]
\begin{lstlisting}{ocaml}
type bst = Node of bst * (int[@collect]) * bst | Leaf
[@@satisfying increasing]

let rec insert (x : int) (bt : bst) : bst =
  match bt with
  | Leaf -> Node (Leaf, x, Leaf)
  | Node (l, x', r) ->
      if x < x' then Node(insert x l, x', r) else Node(l, x', insert x r)
\end{lstlisting}
\caption{An OCaml program that manipulates binary search trees\label{fig:bst}}
\end{figure}

\begin{figure}[h]
\begin{lstlisting}{ocaml}
let () =
  let generator rs =
    let x1 = QCheck.Gen.int rs in
    let x2 =
      let rec of_arbogen_bst arbg queue rs =
        Arbogen.(
          match arbg with
          | Tree.Label ("bst", [Tuple []; child]) -> (
            match child with
            | Tree.Label ("Node", [x1; x2; x3]) ->
                let x1, x2, x3 =
                  let x1 = of_arbogen_bst x1 queue rs in
                  let x2 = Testify_runtime.Arbg.to_int x2 queue rs in
                  let x3 = of_arbogen_bst x3 queue rs in
                  (x1, x2, x3)
                in
                Node (x1, x2, x3)
            | Tree.Label ("Leaf", []) -> Leaf
            | x -> failwith "Ill-formed arbogen tree" )
          | x -> failwith "Ill-formed arbogen tree")
      in
      let wg =
        let open Arbogen.Boltzmann.WeightedGrammar in
        { names= [|"bst"; "Node"; "Leaf"; "@collect"|]
        ; rules=
            [| Union
                 [ (0.499977638879, Product [Z 1; Ref 1])
                 ; (0.500022361122, Product [Z 1; Ref 2]) ]
             ; Product [Ref 0; Ref 3; Ref 0]
             ; Z 0
             ; Z 0 |] }
      in
      let tree = Testify_runtime.Arbg.generate wg "bst" rs in
      let nb_collect = Testify_runtime.Arbg.count_collect tree in
      let queue =
        (fun n -> [|Testify_runtime.Sicstus.increasing_list n|]) nb_collect
      in
      of_arbogen_bst tree queue rs
    in
    let rec print_bst = function
      | Node (x1, x2, x3) ->
          "Node"
          ^ ( "("
            ^ (print_bst x1 ^ ", " ^ string_of_int x2)
            ^ ", " ^ print_bst x3 )
          ^ ")"
      | Leaf -> "Leaf"
    in
    let x3 = insert x1 x2 in
    ( x3
    , (("(insert " ^ string_of_int x1 ^ " " ^ print_bst x2) ^ ")")
      ^ " = " ^ print_bst x3 )
  in
  Testify_runtime.(
    add_fun 0x2710 "insert"
      "File \"examples/recursive/bst.ml\", lines 4-8, characters 0-75"
      (opt_print snd) (opt_gen generator)
      (sat_output
         (let open Operators in
         let rec collect_bst n = function
           | Node (x1, x2, x3) ->
               (fun n (x1, x2, x3) ->
                 List.flatten
                   [ collect_bst n x1
                   ; (if n = 0 then Collect.int n else fun x -> []) x2
                   ; collect_bst n x3 ] )
                 n (x1, x2, x3)
           | Leaf -> []
         in
         fun x -> increasing ((collect_bst 0) x)) ))

let () = Testify_runtime.run_test ()
\end{lstlisting}
\caption{Test generated for the function insert\label{fig:bst-generated-code}}
\end{figure}

\section{Type definitions for the Types used in Section~\ref{sec:bench}\label{app:types}}
\begin{figure}[h]
\begin{lstlisting}{ocaml}
type increasing_list =
  | Nil 
  | Cons of ((int)[@collect ]) * increasing_list 
[@@satisfying increasing]

type assoc_list =
  | Nil 
  | Cons of ((int)[@collect ]) * int * assoc_list
[@@satisfying alldiff]

type bicollect = 
  | Empty
  | Cons of (int[@collect 1]) * (int[@collect 2]) * bicollect
[@@satisfying fun x -> increasing x 1 && increasing x 2]

type binary_tree = 
  | Node of binary_tree * (int[@collect]) * binary_tree
  | Leaf
[@@satisfying increasing]

type map = 
  | Node of map * (int[@collect]) * int * map
  | Leaf
[@@satisfying increasing]

type quad_tree_x =
  | LeafX
  | NodeX of
      (int[@collect 1])
      * quad_tree_y
      * quad_tree_y
      * (int[@collect 2])
[@@satisfying fun x -> increasing x 1 && increasing x 2]
and quad_tree_y =
  | LeafY
  | NodeY of
      (int[@collect 3])
      * quad_tree_x
      * quad_tree_x
      * (int[@collect 4])
[@@satisfying fun x -> increasing x 3 && increasing x 4]
\end{lstlisting}
\caption{Constrained Types Used in Experiments }
\end{figure}
